Theoretical study of interacting electrons in one dimension - ground states and experimental signatures

This dissertation focuses on a theoretical study of interacting electrons in one dimension. The research elucidates the ground state (zero temperature) electronic phase diagram of an aluminum arsenide quantum wire which is an example of an interacting one dimensional electron liquid. Using one dimensional field theoretic methods involving abelian bosonization and the renormalization group we show the existence of a spin gapped quantum wire with electronic ground states such as charge density wave and singlet superconductivity. The superconducting state arises due to the unique umklapp interaction present in the aluminum arsenide quantum wire bandstructure discussed in this dissertation. It is characterized by Cooper pairs carrying a finite pairing momentum. This is a realization of the Fulde-Ferrell-Larkin- Ovchinnikov state which is known to lead to inhomogeneous superconductivity. The dissertation also presents a theoretical analysis of the finite temperature single hole spectral function of the one dimensional electron liquid with gapless spin and charge modes (Luttinger liquid). The hole spectral function is measured in angle resolved photoemission spectroscopy experiments. The results predict a kink in the effective electronic dispersion of the Luttinger liquid. A systematic study of the temperature and interaction dependence of the kink provides an alternative way to detect spincharge separation in one dimensional systems where the peak due to the spin part of the spectral function is suppressed.

==> bibliography.tex <==
%
%  bibliography.tex   2004.03.28  15:19:31   Mark Senn <mark@purdue.edu>
%
%  This is the bibliography for the thesis.
%

\bibliography{all}

@article{Kimura, author = {Takashi~Kimura}, journal = prb, volume =
64, pages = {233306}, year = 2001, title = {Conductance
renormalization and conductivity of a multisubband
Tomonaga-Luttinger model}, annote = {multiple subband quantum wire}
}

@article{kimurapair,
   author    = {T.~Kimura and K.~Kuroki and H.~Aoki},
   title     = {Pairing correlation in the three-leg Hubbard ladder-renormalization group and quantum Monte Carlo studies},
   journal   = {J.~Phys.~Soc.~Jpn.},
   pages     = {1377-1390},
   year      = 1998,
   volume    = 67
}
@article{spingap,
   author    = {V.~J.~Emery and  S.~A.~Kivelson and O.~Zachar},
   title     = {Spin-gap proximity effect mechanism of high-temperature superconductivity},
   journal   = prb,
   pages     = {6120-6147},
   year      = 1997,
   volume    = 56
} @BOOK{Starykh,
   author = "Oleg A. Starykh and Dmitrii L. Maslov and Wolfgang Hausler and Leonid I. Glazman",
   title ="Interactions and Quantum Transport Properties of Lower Dimensional Systems, Lecture Notes in Physics,",
   publisher = "Springer",
   year = "2000"
}
@BOOK{concepts,
editor = "K.H. Bennemann and J.B. Ketterson",
author = "E. W. Carlson and V. J. Emery and S. A. Kivelson and D. Orgad",
title = "Concepts in High Temperature Superconductivity in The Physics of Conventional and
Unconventional Superconductors, Vol. II ed.",
publisher ="Springer-Verlag",
year = 2004}


@ARTICLE{Yacoby,
   author = "A. Yacoby and H.L.Stormer and Ned S.Wingreen and L.N.Pfeiffer and K.W.Baldwin and K.W.West",
   year = "1996",
   journal = "Phys. Rev. Lett. ",
   volume = "77",
   pages = "4612"
}
@ARTICLE{Haldane,
   author = "F.D.M.Haldane",
   year = "1981",
   journal = "J.Phys.C:Solid State Phys",
   volume = "14",
   pages = "2585"
} @BOOK{Giamarchi,
      author = "T. Giamarchi",
      title ="Quantum Physics in One Dimension",
      publisher = "Clarendon Press, Oxford",
      year = 2004
} @ARTICLE{Giam_Schulz,
   author = "T. Giamarchi and H.J.Schulz",
   year = "1989",
   journal = "Phys. Rev. B",
   volume = "39",
   pages = "4620"
} @ARTICLE{Schulz,
   author = "H.J.Schulz",
   year = "1996",
   journal = "Phys. Rev. B",
   volume = "53",
   pages = "R2959"
}
} @ARTICLE{Lin,
   author = "H. H. Lin and Leo Balents and Mathew P. Fisher",
   year = "1998",
   journal = "Phys. Rev. B",
   volume = "58",
   pages = "1794"
}
} @MISC{Moser,
   author = "Joel Moser and S.Roddaro and D.Schuh and M.Bichler and V.Pellegrini and G.Abstreiter and M.Grayson",
   note ="to be  published"

}
@MISC{JM,
   author="Joel Moser and T.Zibold and S.Roddaro and D.Schuh and M.Bichler  and V.Pellegrini and G.Abstreiter and M.Grayson",
   year = "2005",
   journal = "Appl. Phys. Lett.",
   volume = "87",
   pages = "052101"
}
 @ARTICLE{Fabrizio,
   author = "M.Fabrizio",
   year = "1993",
   journal = "Phys. Rev. B",
   volume = "48",
   pages = "15838"
} @ARTICLE{Miranda,
   author = "E.Miranda",
   year = "2003",
   journal = "Braz. Jour. Phys.",
   volume = "33",
   pages = "3"
} @MISC{comment, note = "$K_{\sigma}=1 \Rightarrow K^{\pm}_{\sigma}=1$ under the condition
$\frac{b^{int}_{2}}{b^{int}_{1}} \rightarrow$ 0"
}
@MISC{semiclassical, note = "Consider the interaction $t(\cos[\sqrt{4\pi}\phi]+ \cos[\sqrt{4\pi}\theta])$ where
$\phi,\theta$ are order-disorder variables.If neither field ordered the energy would be zero. But we observe
that by gapping either one of the two fields the energy would be -t and hence lowered. Therefore, with dual
fields present definetly one of them will be gapped."
}
@MISC{galilean, note = "The Galilean invariant Luttinger parameter for the spinless case is given by
$K_{\rho}= \sqrt{\frac{1+\frac{U(2k^{o}_{F})}{2\pi
v_{\rho}}}{1+\frac{2U(0)-U(2k^{o}_{F})}{2\pi v_{\rho}}}}$"}
@ARTICLE{Khveshchenko,
   author = "D.V. Khveshchenko and T.M.Rice",
   year = "1992",
   journal = "Phys. Rev. B",
   volume = "50",
   pages = "252"
}

@ARTICLE{Oron,
   author = "O. Zachar",
   year = "2001",
   journal = "Phys. Rev. B",
   volume = "63",
   pages = "205104"
}@ARTICLE{Kusmartsev,
   author = "F.V.Kusmartsev and A.Luther and A.A.Nersesyan",
   year = "1992",
   journal = "JETP Lett.",
   volume = "55",
   pages = "692"
} @ARTICLE{Nersesyan,
   author = "A.A.Nersesyan and A.Luther and F.V.Kusmartsev",
   year = "1993",
   journal = "Phys. Lett. A",
   volume = "176",
   pages = "363"
}
 @ARTICLE{Yakovenko,
   author = "V.M.Yakovenko",
   year = "1992",
   journal = "JETP Lett",
   volume = "56",
   pages = "5101"
}
@ARTICLE{Arrigoni,
   author = "E. Arrigoni and S.A.Kivelson",
   year = "2003",
   journal = "Phys. Rev. B",
   volume = "68",
   pages = "180503"
}
@BOOK{Gogolin,
      author = "Alexander O. Gogolin and Alexander A. Nersesyan and Alexei M. Tsvelik",
      title ="Bosonization and Strongly Correlated Systems",
      publisher = "Cambridge University Press",
      year = 1998
}

@ARTICLE{Dagotto, author="E.Dagotto", year="1999", journal="Rep.
Prog. Phys.", volume="62", pages="1525" }

@ARTICLE{ Orignac, author="E.Orignac and T.Giamarchi",
year="1997",journal="Phys. Rev. B", volume="56",pages="7167"}

@ARTICLE{ Finkelstein, author="A.M.Finkelstein and A.I.Larkin",
year="1993", journal="Phys. Rev. B", volume="47", pages="10461"}

@ARTICLE{Nagaosa, author="N.Nagaosa", year="1995", journal="Solid
State Commun", volume="94",pages="495"}

 @ARTICLE{Balents,
   author = "L.Balents and M.P.A.Fisher",
   year = "1996",
   journal = "Phys. Rev. B",
   volume = "53",
   pages = "12133"
}

 @ARTICLE{Shelton,
   author = "D.G.Shelton and A.M.Tsvelik",
   year = "1996",
   journal = "Phys. Rev. B",
   volume = "53",
   pages = "14036"
}

 @ARTICLE{Riera,
   author = "E.Dagotto and J.Riera and D.Scalapino",
   year = "1992",
   journal = "Phys. Rev. B",
   volume = "45",
   pages = "5744"
}

@ARTICLE{Noack,
   author = "R.Noack and S.White and D.Scalapino",
   year = "1994",
   journal = "Phys. Rev. Lett.",
   volume = "73",
   pages = "882"
}

@ARTICLE{Poilblanc,
   author = "D.Poilblanc and H.Tsunetsugu and T.M.Rice",
   year = "1994",
   journal = "Phys. Rev. B",
   volume = "50",
   pages = "6511"
}

@ARTICLE{Tsunetsugu,
   author = "H.Tsunetsugu and M.Troyer and T.M.Rice",
   year = "1994",
   journal = "Phys. Rev. B",
   volume = "49",
   pages = "16078"
}

@ARTICLE{White,
   author = "S.R.White and I.Affleck and D.J.Scalapino",
   year = "2002",
   journal = "Phys. Rev. B",
   volume = "65",
   pages = "165122"
}

@ARTICLE{Varma,
   author = "C.M.Varma and A.Zawadowski",
   year = "1985",
   journal = "Phys. Rev. B",
   volume = "32",
   pages = "7399"
}

@BOOK{Devreese,
      editor = "J.T.Devreese",
      title ="Highly Conducting One Dimensional Solids",
      publisher = "Plenum Press, New York",
      year = "1997"
}

@ARTICLE{Apel,
   author = "W.Apel and T.M.Rice",
   year = "1992",
   journal = "Phys. Rev. B",
   volume = "26",
   pages = "7063"
}
@ARTICLE{Kane,
   author = "C.L.Kane and M.P.A.Fisher",
   year = "1992",
   journal = "Phys. Rev. Lett.",
   volume = "68",
   pages = "1220"
}

@ARTICLE{Fisher,
   author = "C.L.Kane and M.P.A.Fisher",
   year = "1992",
   journal = "Phys. Rev. B",
   volume = "46",
   pages = "15233"
}

@ARTICLE{Pfeiffer,
   author = "L.N.Pfeiffer and H.L.Stormer and K.W.Baldwin and K.W.West and A.R.Goni and A.Pinczuk and R.C.Ashoori
   and M.M.Dignam and W.Wegscheider",
   year = "1993",
   journal = "J. Crys. Growth",
   volume = "849",
   pages = "127"
}


@ARTICLE{Motohisa,
   author = "J.Motohisa and H.Sakaki",
   year = "1992",
   journal = "Appl. Phys. Lett.",
   volume = "63",
   pages = "1786"
}

@ARTICLE{Kurdak,
   author = "C.Kurdak and A.Zaslavsky and D.C.Tsui and M.B.Santos and M.Shayegan",
   year = "1995",
   journal = "Appl. Phys. Lett.",
   volume = "66",
   pages = "323"
}

@ARTICLE{Stone,
   author = "D.L.Maslov and M.Stone",
   year = "1995",
   journal = "Phys. Rev. B",
   volume = "52",
   pages = "R5535"
}
@ARTICLE{Safi,
   author = "I.Safi and H.J.Schulz",
   year = "1995",
   journal = "Phys. Rev. B",
   volume = "52",
   pages = "R17040"
}
@ARTICLE{Ponomarenko,
   author = "V.V.Ponomarenko",
   year = "1995",
   journal = "Phys. Rev. B",
   volume = "52",
   pages = "R8666"
}
@ARTICLE{Maslov,
   author = "D.L.Maslov",
   year = "1995",
   journal = "Phys. Rev. B",
   volume = "52",
   pages = "R14368"
}
@ARTICLE{Yaroslav,
   author = "Y.Tserkovnyak and B.I.Halperin and O.M.Auslaender and A.Yacoby",
   year = "2002",
   journal = "Phys. Rev. Lett.",
   volume = "89",
   pages = "136805"
}


